Machine Learning Methods for Shark Detection

This essay reviews human observer-based methods employed in shark spotting in Muizenberg Beach. It investigates Machine Learning methods for automated shark detection with the aim of enhancing human observation. A questionnaire and interview were used to collect information about shark spotting, the motivation of the actual Shark Spotter program and its limitations. We have defined a list of desirable properties for our model and chosen the adequate mathematical techniques. The preliminary results of the research show that we can expect to extract useful information from shark images despite the geometric transformations that sharks perform, its features do not change. To conclude, we have partially implemented our model; the remaining implementation requires dataset.

==> chapter11.tex <==
\chapter{Introduction}
In Machine Learning problems, classification is considered as the main and most used task and attracts many researchers. For our work, we use Machine Learning techniques to solve classification task related to one problem in South Africa, precisely in Capetown.

In Capetown, people during public holidays, school holidays, weekends and even open days use to spend times in surfing alone or with their family at the different beaches (Muizenberg, Fish Hoek, Kosel Bay, etc$\cdots$). The danger that can be arisen is the presence of shark that can cause deaths (Figure \ref{fig:probl3}). Nevertheless, people prefer to come and enjoy their times at the beaches as shown in Figure \ref{fig:probl1}.
\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.31\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/beach}
        \caption{Muizenberg Beach}
        \label{fig:probl1}
    \end{subfigure}
   \begin{subfigure}[b]{0.31\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/contact}
        \caption{shark spotter}
        \label{fig:probl2}
    \end{subfigure}
    \begin{subfigure}[b]{0.31\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/attacks}
        \caption{shark attack}
        \label{fig:probl3}
    \end{subfigure}
    \caption{shark spotter}
    \label{fig:problem}
\end{figure}

In 2004, a program sharkspotters(\href{http://sharkspotters.org.za/}{shark spotters}) came up with objective to control the presence of shark in the ocean while people are surfing. The spotters (see Figure \ref{fig:probl2}) in the case of Muizenberg beach, stand on the mountain watching over through binoculars, a specific surface on the ocean  in which surfers could not go out of. The spotters on the mountain are in communication with others spotters on the beach. However, there are four types of flags that spotters use to communicate with surfers. The four flags transmit the following messages: (1) \textit{Green flag}: the conditions are good for spotters to work. (2) \textit{Black flag}: the conditions are poor for spotters to perform a good work. (3) \textit{Red flag}: be warned, shark is in the water. (4) Finally, the \textit{White flag} which asks to surfers to leave immediately water in order to avoid the risk of death as shown in Figure \ref{fig:probl3}.

Poor condition is the interest of this work. While we were holding the interview with spotters, we have understood that the poor conditions are mentioned when it is raining, in the presence of murky or rough weather, when it is cloudy or windy. Consequently, two risks could happen: (1) \textbf{False Positive}: spotters could ask surfers to leave immediately the ocean because shark is spotted while it is not really a shark. When that happens several times, suffers will no longer trust spotters. Then it is the first danger. (2) \textbf{False Negative}: spotters could not see a shark while there is one in the ocean. This is the second danger. Therefore, the purpose of this work is to propose an automatised system supporting human decision, i.e. when a suspect object is spotted, an image is taken and both human and automatised system classify the object whether is shark or not, compare the results and take decision. In other words, we need to reduce the risks of False Positive and False Negative by converting the actual manual sharkspotter program to a semi-automatic sharkspotter.
We aim to enhance shark detection by designing an automatised system able to: (1) Detect shark despite all geometric transformations it can perform. (2) Detect shark despite the climate or weather. (3) Recognize shark from image.

%Hypotheses
The shark spotting problem involves three main steps: $(1)$ Detect a suspect image in water. $(2)$ Decide whether or not is a shark. $(3)$ Deliver a message to surfers in case of shark. Throughout this work, the following questions will be answered: $(1)$ How to come up with a model in which we can trust. $(2)$ How to extract useful information from an image. $(3)$ How to combine different classification techniques and improve the output. We assume that data we will use is not linear separable and the image to be classified contains objects related to ocean (fish, shark, people, water). 

From Machine Learning point of view, shark spotting is considered as a classification task where we need to classify four objects: shark, shark school, baby shark and other objects in the ocean. It is really a multi-class classification task. The choice of four classes is chiefly motivated by the risk that would be caused not only at the nearest beach of the points where shark school is detected but also at all the beaches surrounding. Likely the risk of baby shark is less considerable than the risk of mature shark. Since the actual program gives a good result apart from the poor conditions mentioned above, we need really to come up with an accurate model that could support the existing system. As for the actual research [\cite{DSF1}] looking for how to combine different classification techniques in order to improve their outputs, we are willing to base on fusion technique whereby the different techniques used are based on different approaches. Truly their combination will preserve their strength and reduce their weaknesses. Their descriptions are given in the following chapters but behold that there are some pretreatment techniques to use in order to prepare images before classifying, i.e. to reduce noise and improve image contrast due to weather, detect different shapes in image and to extract useful information and reduce image size.

Different features extractors might focus on different types of data, for example moment-based and frequency-based. We aim to combine features extractors outputs in order to get a diversity of features for use in classification. Therefore, the Generic Fourier Descriptor will be used as feature frequency based and the Complex Moment and Legendre Moment are used as features moment-based. The choice of the two feature moment-based is motivated to the fact that one constructs an orthogonal set of features while the other does not. 

Artificial Neural Network (ANN) is used as the first mathematical model for classification; this approach trains classifier from training data so that it can assign a new image to the class using its knowledge, i.e. it evaluates the training error based on inputs and minimizes it. ANN is inspired of human nervous system. The human system is based on \textit{neuron} which processes information. A neuron receives information sent by another neuron through its \textit{dendrites} and sends the information to others neurons using its \textit{axon}[\cite{ANN1}]. The second classification technique used is K-Nearest Neighbours which evaluates the similarity between the query image and the rest of training data, looks for $k$ images that are very close to the query image and proceeds by voting, i.e. a query image $x_q$ is assigned to class $c_k$ having more images among $k$ images chosen [\cite{KNN1}].
Conversely, the last classification technique, Support Vector Machine (SVM) works by reducing the classification error, i.e. defines classification error on the results followed by its minimization. SVM transforms a non-linear problem to a linear problem by the use of kernel trick, converges to a global minimal since the problem is converted to a convex problem. Dempster-Shafer Fusion (DSF) is used to combine classifiers outputs and considers the uncertainties and combining different sources of evidence[\cite{DSF2}].

%layout of the work
The rest of the work is  organized as follows: Chapter 2 presents a consistent list of properties required for a classification to perform a good output and the mathematical analysis made for a relevant choice of techniques to use. Chapter 3 shows the different preliminary tasks applied in image such as geometric transformations in order to extract its useful information. Chapter 4 presents the three classifications approaches used and how they are combined in order to improve the output. Chapter 5 presents results obtained and discussion made. Finally conclusion and further work are presented.
